Bi-level regularization via iterative mesh refinement for aeroacoustics

In this work, we illustrate the connection between adaptive mesh refinement for finite element discretized PDEs and the recently developed \emph{bi-level regularization algorithm}. By adaptive mesh refinement according to data noise, regularization effect and convergence are immediate consequences. We moreover demonstrate its numerical advantages to the classical Landweber algorithm in term of time and reconstruction quality for the example of the Helmholtz equation in an aeroacoustic setting.

==> content.tex <==
\def\R{\mathbb{R}}
\def\C{\mathbb{C}}
\def\N{\mathbb{N}}
\def\F{\mathbb{F}}
\def\Om{\Omega}
\def\Ls{L^2(\Omega_0)}
\def\Ld{L^2(\Omega_1,\C)}
\renewcommand{\Re}{\mathop{Re}\nolimits}
\renewcommand{\d}{\,\mathrm{d}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\section{Inverse aeroacoustic source with Helmholtz equation} We investigate an inverse source problem in aeroacoustics, where an unknown source $\phi$  is located in the sub-region $\Omega_0$ of an enclosed room, denoted by $\Omega$, and needs to be determined from acoustic oscillations measured outside of $\Omega_0$. The measurement region, denoted $\Omega_1\subset\Omega$, includes a finite number of obstacles, e.g.~sound-hard walls, reflecting the sound wave propagating to the aeroacoustic sensors \cite{aeroacoustic}. $\Omega$ is treated as a homogeneous medium, enabling the Helmholtz equation to adequately model the oscillation at a single frequency and constant sound speed.

Mathematically, let the room $\Omega$ be a bounded Lipschitz domain in $\R^d$, $d=1,2,3$; for illustration in this article, we choose $d=2$. The unknown real source
\begin{align}
\phi\in \Ls \qquad \Omega_0\subset\text{int }\Omega
\end{align}
generates a complex wave field $u$, propagating throughout the room. The measurement region $\Om_1\subset\Om$ is disjoint from the source domain $\Om_0$ in the sense that $\overline{\Om_0}\cap\overline{\Om_1}=\emptyset$; we here assume that $\Om_1$ additionally contains three disjoint rectangular sound-hard scatterers $S_i$, $i\in\{1,2,3\}$; see Section \ref{sec:num}. We then define the measurement operator with $\Omega_1:=\Omega\setminus\big(\Omega_0\cup\bigcup_{i=1}^3S_i\big)$ as
\begin{equation}\label{data}
\begin{split}
M: &\, H^1(\Omega\setminus\bigcup_{i=1}^3S_i,\C)\to  L^2(\Omega_1,\C)\qquad u\mapsto u|_{\Omega_1}
\end{split}
\end{equation}
 
Acoustic wave traveling in the room at a constant wave number $k\in\R$ is governed by the homogeneous Helmholtz equation 
\begin{alignat}{2}\label{eq}
&\Delta u + k^2 u  = \phi &&\text{in $\Omega\setminus\bigcup_{i=1}^3S_i$},\\
\frac{\partial u}{\partial n} & = ik u \quad \text{on \,$\partial \Omega$,} \qquad
&&\frac{\partial u}{\partial n}  = 0 \quad \text{on \,$\bigcup_{i=1}^3\partial S_i$,} \nonumber
\end{alignat}
where $\phi$ is implicitly extended by zero outside of $\Omega_0$. The sound-hard scatterers are modeled by the Neumann condition on the interior Lipschitz boundaries $\partial S_i$, and on the exterior boundary $\partial\Omega$, we use an approximate Sommerfeld radiation condition; $n$ are the outward normal vectors.

The linear source-to-observable map $F$ is defined by
\begin{align}
F: \Ls\to\Ld  \qquad \phi \mapsto u|_{\Omega_1};
\end{align} 
hence, we formulate the inverse aeroacoustic source problem given noisy data $y^\delta$ as
\begin{align*}
\text{Find } \phi: \quad F(\phi)=y^\delta.  %\quad\text{s.t.}\quad u \text{ solves } \eqref{eq}.
\end{align*}

We remark that while the PDE \eqref{eq} is well-posed
\cite{ColKre13}, the observation operator $M$ renders $F$ non-injective and compact, making the inverse problem ill-posed. Thus, regularization is required to stably reconstruct the unknown acoustic source. 

We shall use the bi-level regularization scheme \cite[Algorithm 1.2]{nguyen24} for the reconstruction process. Here, the author proposes a novel bi-level inversion framework, in which the upper level-iteration for the unknown parameter -- here, the source term -- embeds a lower-iteration solving nonlinear PDEs inexactly. A key contribution of \cite{nguyen24} is the derivation of stopping rules for upper- and lower-level that can ensure convergence. In addition, embedding any PDE solver (FD, FEM, multigrid etc.)~into the lower-level, the error analysis in \cite{nguyen24} can inform an adaptive discretization scheme via multi-grid size, -mesh size or -resolution \cite{Trottenberg} that are computationally effective by not fixing a single fine scale in the inversion process.

As the model \eqref{eq} is rather classical, we shall not use the lower-level to approximate $u$, instead implementing a FEM solver with an adaptive \underline{mesh refinement} strategy suggested in \cite[Theorem 2]{nguyen24} to speed up the reconstruction, while, crucially, maintaining the regularizing property. This forms the contribution of this article. 

\section{Inversion algorithm with mesh iterative refinement}
In \cite[Algorithm 1.2]{nguyen24}, the upper-level iteratively updates the source term, and requires the adjoint of the source-to-observation $F$ to be derived.
\begin{lemma}[Adjoint]
The Hilbert space adjoint $F^*:\Ld \mapsto \Ls$ is
\begin{equation}\label{adjoint}
\begin{split}
F^*v:=\Re(z)|_{\Omega_0} \qquad&\text{ with}\\
\Delta z + k^2 z  = v \qquad&\text{in $\Omega\setminus\bigcup_{i=1}^3S_i$}, \\
\frac{\partial z}{\partial n} = -ik z \quad\text{on $\partial \Omega$,}\qquad&
\frac{\partial z}{\partial n}  = 0 \quad\text{on $\bigcup_{i=1}^3\partial S_i$,} 
\end{split}
\end{equation}
where $v$ is implicitly extended by zero outside of $\Omega_1$.
\end{lemma}
\begin{proof}
For any $\phi\in \Ls, v\in \Ld$, we write the inner product
\begin{align*}
\left(F\phi,v\right)_{\Ld}&:=\Re\int_{\Omega_1}u|_{\Omega_1}\overline{v}\,dx=Re\int_{\Omega_0\cup\Omega_1}u\, \overline{v}\,dx\\
&=Re\left(\Delta u+k^2u,z\right)_{L^2(\Omega_1\cup\Omega_0,\C)} + Re\left(iku-\partial_n u,z\right)_{L^2(\partial \Omega,\C)}\\
&=\left(\phi,\Re(z)\right)_{L^2(\Omega_1\cup\Omega_0)} =\left(\phi,\Re(z)|_{\Omega_0}\right)_{\Ls}\quad=:\left(\phi,F^* v\right)_{\Ls}
\end{align*}
where $\overline{(\cdot)}$ denotes the complex conjugate. The proof is complete.
\end{proof}

%\begin{remark}[Unique identifiability] Data collected by the measurement $M$ designed in \eqref{data} suffices to uniquely recover the unknown source. Indeed, for two wave fields $u,v$ that coincide in the measurement region, their difference $u-v$  solves \eqref{eq}. \blue{Check} The unique continuation principle \blue{Evans} implies vanishing of the difference field in the whole room, thus the two associated sources are identical.
%\end{remark}


\begin{remark}[Multi grid size]We here remark how \cite{nguyen24} applies to multi-grid and mesh refinement. Given data noise $\delta$, \cite[Proposition 5]{nguyen24} shows that for each upper-iteration $j$, the lower-iteration should be run with precision $\epsilon_j=\delta/q^j$, $q\geq 1$, terminating the upper-level at the stopping index $j^*(\delta,q)$ according to \cite[Theorem 2]{nguyen24}. In this study, the lower-level discretization/approximation error $\epsilon_j$ translates to the FEM grid size $h_j$, where for any FEM its grid size $h$ is approximately given as $h\approx\max\left(2\int_E1\d x\right)^{1/2}$, the max being taken over elements $E$ of the FEM, approximately yielding the max height of any triangle in the mesh discretization. By \cite{BrennerScott}, the approximation error of the FEM is proportional to $h$, that is, $\epsilon = Ch$ for some $C$. By this analysis, the grid size is initially kept constant $\epsilon_0:=Ch_0>0$, and must be iteratively refined as soon as $j\geq (\ln\delta - \ln Ch_0)/\ln q$; we adaptively refine the mesh in all elements corresponding to large $h$. Expressed as an algorithm, we have \label{rem:multi}
\end{remark}

\vspace{-0.75cm}

\begin{algorithm}
\label{alg:cap}
\begin{algorithmic}
%\Require $j \geq 0$
\Ensure $\phi^0:=0$, \text{step size }$\mu$, \text{threshold }$\tau$
\While{$\|y^\delta-F\phi^j\|_2 \leq \tau\delta$}
\If{$j \geq (\ln\delta - \ln Ch_0)/\ln q$}
    \State refine mesh as in Remark \ref{rem:multi}
\EndIf
\State $v\gets F_{h(\delta,j)}\phi^j - y^\delta$
\State $z \gets$ solves \eqref{adjoint} \text{ with } $F^*_{h(\delta,j)}$, $v$
\State $\phi^{j+1} \gets \phi^j - \mu z$
\EndWhile
\end{algorithmic}
\end{algorithm}
\vspace{-1.5cm}

\section{Numerical experiments}\label{sec:num}

In this Section, we numerically verify our analysis by reconstruction of the source 
\vspace{-0.2cm}
\[
\phi(x,y):=
\sqrt{\min\{
\tfrac{1}{4}-x^2-y^2, 0
\}}
\cos\left(
2\pi\sqrt{x^2+y^2}
\right).
\]
\vspace{-0.5cm}

\begin{wrapfigure}{l}{0.449\textwidth}
\vspace{-0.6cm}
\centering
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_1}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_2} \\[-1ex]
%\centering
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_3}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_4}
\vspace{-0.65cm}
\caption{Iterative reconstruction on each mesh in the bi-level algorithm, prior to refinement. Noise level $1\%$. $h\approx 0.531$, $0.265$, $0.139$, $0.08$.}
\vspace{-0.6cm}
\end{wrapfigure}

For the approximate PDE solver, we employ the NGSolve \cite{Schoberl} finite element method (FEM) package to create a discretization of our domain $\Omega:=[-1,1]^2\subset\R^2$ and subsequently also the forward operator $F$, where we have chosen $\Omega_0:=[-1/2,1/2]^2\subset\Omega$ and $\Omega_1:=[-1,1]^2\setminus [-11/20,11/20]^2\subset\R^2$ (see Figures; sound-hard scatterers $S_i$, $i=1,2,3$ are as modeled). We approximate the true state $u:=F\phi$ by applying a finely discretized FEM solver ($h^\dagger\approx 0.046$), and conduct two numerical comparisons for the recovery of $\phi$ from noisy observations $y^\delta$, where $y^\delta-u$ consists of additive Gaussian white noise $\delta$ of relative size $1\%$ resp.~$10\%$ relative to $u$. In both experiments, two methods of recovering $\phi$ are compared.

\begin{wrapfigure}{r}{0.449\textwidth}
\vspace{-0.5cm}
\centering
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_bil}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_001_dir} \\
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_nomesh}
\vspace{-0.3cm}
\caption{Left: Output of bi-level. Right: Output of direct Landweber. Bottom: True source $\phi$. $1\%$ noise, mesh not depicted.}
\vspace{-2.9cm}
\end{wrapfigure}

The first method is the bi-level Landweber iteration with mesh refinement as proposed above, beginning with a coarse mesh ($h_0\approx 0.531$), $q:=2^{1/60}$ and $C:=1.4/\delta$. The second method is \enquote{direct} Landweber regularization, carried out %as $\phi^{j+1} := \phi^j - \mu F^*(F\phi^j - y^\delta)$, $\phi^0 := 0$, $j\in\N_0$ 
on a single, distinct FEM-discretized mesh that is finer than any used by the bi-level and coarser than the FEM used to generate the approximate state $u$ ($h_{\text{direct}}\approx 0.064$). In all cases, $\mu$ was estimated as $\mu\approx 0.075$, and all iteration was stopped at the first (upper-)index $j$ satisfying the discrepancy principle $\|y^\delta-F\phi^j\|_2 \leq \tau\delta$ with $\tau:=1.3$.

\begin{wrapfigure}{l}{0.449\textwidth}
%\centering
\vspace{-0.5cm}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_010_1}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_010_2}
\vspace{-0.5cm}
\caption{Iterative reconstruction on each mesh in the bi-level algorithm, prior to refinement. Noise level $1\%$. $h\approx 0.531$, $0.265$.}
\vspace{-0.5cm}
\end{wrapfigure}

We make some remarks regarding the reconstruction. Figure \ref{fig:errs} displays the reconstruction errors and residuals for the two methods, plotted by total time taken. This includes time required for mesh refinement (bi-level only), for the Landweber step and for computation of the residual. 

%Figure \ref{fig:errs} show the numerical outputs of the two experiments, showing relative reconstruction error $\|\phi-\phi^j\|_2/\|\phi\|_2$ (top) and residual $\|u-F\phi^j\|_2/\|u\|_2$ over \emph{time} on the $x$-axis, in seconds, of the bi-level algorithm (blue resp.~red for reconstruction error resp.~residual) and for the direct Landweber (black dashed line in both cases). The 

For both $1\%$ and $10\%$ relative noise, the bi-level algorithm reached the discrepancy principle much earlier than the direct Landweber algorithm. In both cases, the final residual was smaller for the bi-level algorithm than for the direct Landweber algorithm. For $1\%$ relative noise, the final reconstruction for the direct Landweber method was slightly better than that of the bi-level algorithm, but the latter reached a higher precision much earlier despite undergoing three mesh refinements, and was only overtaken after a longer period of time. For $10\%$ relative error, the bi-level algorithm outperformed the direct Landweber method in all respects despite needing only one mesh refinement. These observations seem to justify the intuition that higher noise levels can efficiently be handled with coarser grids, an effect that the bi-level method makes explicit.

\begin{figure}[h!]%{l}{0.5\textwidth}
%\centering
\vspace{-0.2cm}
\includegraphics[clip,width=0.49\textwidth,keepaspectratio]{Rec_001}
\includegraphics[clip,width=0.49\textwidth,keepaspectratio]{Res_001} \\[2ex]
\includegraphics[clip,width=0.49\textwidth,keepaspectratio]{Rec_010}
\includegraphics[clip,width=0.49\textwidth,keepaspectratio]{Res_010}
\vspace{-0.1cm}
\caption{Error plots over time. Blue background denotes which mesh refinement the bi-level algorithm is currently on.}%Left: Relative errors. Right: Residuals. Top: $1\%$ relative noise. Bottom: $10\%$ relative noise.}
\vspace{-0.5cm}
\label{fig:errs}
\end{figure}

\subsection*{Conclusions}

\begin{wrapfigure}{r}{0.449\textwidth}
\centering
\vspace{-0.75cm}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_010_bil}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_010_dir}
\includegraphics[trim={19.8cm 5cm 19.8cm 7.1cm},clip,width=0.22\textwidth,keepaspectratio]{f_nomesh}
\vspace{-0.3cm}
\caption{Left: Output of bi-level. Right: Output of direct Landweber. Bottom: True source $\phi$. $10\%$ noise, mesh not depicted.}
\vspace{-1.1cm}
\end{wrapfigure}

In this article, we have demonstrated that the bi-level algorithm produces highly efficient numerical results in a manner consistent with that claimed in \cite{nguyen24}.

%Here, the experimenter can freely control some \emph{design parameter} $w$ controlling the unknown-to-observable map $F_w$, and wishes to choose the design parameter $w$ that leads to the best reconstruction. 
The recent developments in bi-level algorithms \cite{nguyen24,nguyen-seqbi} opens up exciting usage within the field of optimal experimental design (OED). \cite{Aarset} newly proposed a novel, high-speed algorithm for linear OED. As remarked in \cite{Ucinski}, detailed treatment of the non-linear case would require additional developments within bi-level algorithms, which the authors believe may now be available.




